From Real to Complex: Enhancing Radio-based Activity Recognition Using Complex-Valued CSI

Activity recognition is an important component of many pervasive computing applications. Radio-based activity recognition has the advantage that it does not have the privacy concern and the subjects do not have to carry a device on them. Recently, it has been shown channel state information (CSI) can be used for activity recognition in a device-free setting. With the proliferation of wireless devices, it is important to understand how radio frequency interference (RFI) can impact on pervasive computing applications. In this paper, we investigate the impact of RFI on device-free CSI-based location-oriented activity recognition. We present data to show that RFI can have a significant impact on the CSI vectors. In the absence of RFI, different activities give rise to different CSI vectors that can be differentiated visually. However, in the presence of RFI, the CSI vectors become much noisier and activity recognition also becomes harder. Our extensive experiments show that the performance of state-of-the-art classification methods may degrade significantly with RFI. We then propose a number of counter measures to mitigate the impact of RFI and improve the location-oriented activity recognition performance. We are also the first to use complex-valued CSI to improve the performance in the environment with RFI.

==> Tex/method_170114.tex <==
%\vspace{-2mm}
\section{Activity Recognition using CSI}\label{sec:methods}
This section presents our method to recognise a set of activities using CSI in the device-free setting. We first demonstrate that CSI is influenced by activities taking place in a room and can be used to identify the activity. We can present the challenge of CSI based activity recognition when RFI is present. Finally, we present our SRC based classification method which takes the RFI into consideration. 

\subsection{CSI contains activity information}\label{subsec:feasibility}
We first present some intuition on why device-free CSI-based activity recognition is possible. Figure ~\ref{fig:multipathexample} depicts an indoor environment with two wireless nodes and the multi-paths that the radio propagation may take. It shows that different multi-path effects can be obtained if a person is sitting and if a person is standing. This results in different CSI vectors at the receiver and can be used to identify the activity. 

In order to demonstrate the feasibility of CSI-based activity recognition, we set up two WASP nodes in an apartment with one living room and one bedroom. The nodes were 5 metres apart with 3 (???) walls in the line-of-sight path between the nodes. The subject was positioned in an AoI between the two nodes but was not in the direct path between the 2 nodes (???). The subject carried out 4 different activities: sitting, lying, standing and walking. A WASP node is used as the transmitter and the other as a receiver. The transmitter sends a packet of size ??? bytes to the receiver at 10 packets per seconds. For each packet received, the receiver used the WASP interface to obtain the CSI vector and SNR for that packet. It is also important to point out that the data in this experiment was collected in a \emph{clean} environment without any RFI. 

Fig.~\ref{fig:examplefrequencyresponse} shows the normalised CSI vectors under the four different activities. The horizontal axis shows the sample number where a sample corresponds to a packet. There are 320 values in the vertical axis which corresponds to the 320 sub-carriers. The magnitude of the CSI is shown as an heat plot. We have put four blocks of data side-by-side in the figure; the four blocks correspond to the four activities of lying, sitting, standing and walking. It can readily be seen that the four activities have highly distinguishable CSI. This confirms that CSI contains information on activity. Another observation that we can make is that the CSI fluctuates a lot when the subject was walking. This is due to different multi-path effects created by the person walking. Fig.~\ref{fig:examplefrequencyresponse} shows the CSI when a 125MHz bandwidth is used. We now show that the same observations also apply when we use a 20MHz channel. The red box in Fig.~\ref{fig:examplefrequencyresponse} is Channel 157 in the 802.11 standards. We have enlarged the CSI in the red box and plotted it in Fig.~\ref{fig:examplefrequencyresponsecleanpart}. It can be seen that the CSI for the four activities are very distinguishable and walking creates more fluctuations in CSI. 

Fig.~\ref{fig:exampleRSS} shows the SNR of the corresponding samples (packets). It shows that the SNR has a slightly larger fluctuation when the subject was walking. However, there does not appear to be any noticeable differences in the SNR data series among lying, sitting and walking. These observations suggest that it may be possible to use SNR to distinguish between walking from the other three activities where the subject was stationary. However, it does not seem to be possible to use SNR to distinguish between the three stationary activities. 

\begin{figure}[htb]
   \centering
    \includegraphics[scale = .5]{figure/multiple_path_example_c_3.pdf}
    \caption{Examples of multiple paths caused by different activities}\label{fig:multipathexample}
\end{figure}



\begin{figure*}[htb]
{
\centering
       \subfigure[CSI amplitute vector in clean environment]{
        \includegraphics[scale = .3]{figure/Example_frequency_response/Example_frequency_response_c.pdf}
        \label{fig:examplefrequencyresponse}
    }
    \subfigure[CSI vectors of in Channel 157 under RFI]{
            \includegraphics[scale = .3]{figure/Example_frequency_response/Example_frequency_response_clean_part_c.pdf}    
            \label{fig:examplefrequencyresponsecleanpart}
            }
    \subfigure[SNR]{
        \includegraphics[scale = .3]{figure/Example_frequency_response/Example_RSS_c.pdf}    
        \label{fig:exampleRSS}
        }
     \subfigure[CSI vectors in RFI environment]{
             \includegraphics[scale = .3]{figure/Example_frequency_response_noise/Example_frequency_response_noise_whole_c.pdf}
             \label{fig:examplefrequencyresponsenoisewhole}
         }
     	\subfigure[CSI vectors of 802.11 5.8 GHz Channel 157 under RFI]{
             \includegraphics[scale = .3]{figure/Example_frequency_response_noise/Example_frequency_response_noise_part_c.pdf}
             \label{fig:examplefrequencyresponsenoisepart}
         }    
         \subfigure[SNR of under RFI]{
             \includegraphics[scale = .3]{figure/Example_frequency_response_noise/Example_RSS_noise_whole_c.pdf}    
             \label{fig:exampleRSSnoise}
             }    
         \caption{Frequency response and SNR performance in different activities}
               \label{fig:dynamicRSSexample}               
}
\end{figure*} 




%\begin{figure*}[htb]
%{
%\centering
%       \subfigure[CSI vectors in RFI environment]{
%        \includegraphics[scale = .3]{figure/Example_frequency_response_noise/Example_frequency_response_noise_whole_c.pdf}
%        \label{fig:examplefrequencyresponsenoisewhole}
%    }
%	\subfigure[CSI vectors of 802.11 5.8 GHz Channel 157 under RFI]{
%        \includegraphics[scale = .3]{figure/Example_frequency_response_noise/Example_frequency_response_noise_part_c.pdf}
%        \label{fig:examplefrequencyresponsenoisepart}
%    }    
%    \subfigure[SNR of under RFI]{
%        \includegraphics[scale = .3]{figure/Example_frequency_response_noise/Example_RSS_noise_whole_c.pdf}    
%        \label{fig:exampleRSSnoise}
%        }
%         
%         \caption{Frequency response and SNR performance in different activities}
%               \label{fig:dynamicRSSexamplenoise}               
%}
%\end{figure*}

\subsection{Challenges of CSI-based activity recognition} 
The above results were obtained when the two WASP nodes were in a clean environment. We conducted another experiment using the same set up but we added a pair of IEEE 802.11a devices that communicated in Channel 157 (a 20 MHz band). Our goal is to understand the impact of RFI on CSI and SNR.  

Fig.~\ref{fig:examplefrequencyresponsenoisewhole} shows the CSI for the four activities when RFI is present in Channel 157. It shows that the CSI in Channel 157 (enclosed by the red rectangle) is fairly noisy but the four activities still have distinguishable CSI outside of Channel 157. This suggests that if wide-band devices are used to obtain the CSI for activity recognition, then we can use the part of CSI with little RFI to identify the activity. However, wide-band devices such as WASP are not common off-the-shelf devices. We therefore consider the possibility of using the CSI in an interfered channel to perform activity recognition. 

In order to examine the effect of RFI, we plotted the CSI of Channel 157 in Fig.~\ref{fig:examplefrequencyresponsenoisepart}. It shows that the CSI vectors of different activities are no longer highly distinguishable. However, if we look closer at the CSI vectors of each activity, we can see that a number of CSI vectors among one activity are almost the same. This recurrence of CSI vectors suggest that we may use a block of CSI vectors for classification instead of individual CSI vectors. However, this classification is going to be challenging because the CSI vectors appear to be fairly noisy. We will propose a few different classification methods in Section \ref{subsec:ar_with_rfi} to address this challenge. 

We now examine the impact of RFI on SNR. Fig.~\ref{fig:dynamicRSSexample} shows the SNR of the four activities when RFI is present in Channel 157. We see that the SNR of all four activities are highly fluctuating. We suggested earlier that it would be possible to tell walking from the static activities using SNR when RFI is absent, however, this does not appear to be feasible once RFI is present. 

To sum up, it is a challenge to use CSI to perform activity recognition when RFI is present. 

%However, the deviation feature based walking detection has limitation, it cannot take effect under RFI. RFI brings the noise interference, and make the deviation of SNR vary significantly even when  the static activities are conducted. Fig.\ref{fig:dynamicRSSexamplenoise} shows SNR performance under RFI. Because SNR deviation under RFI is also large, it is hard to see any difference between the static activities and walking.
%
%Alternatively, we can only use CSI vectors for fingerprinting the activities. Fig.~\ref{fig:examplefrequencyresponsenoisewhole} shows the CSI vector under RFI of 5.8 GHz 802.11 Channel 157. CSI elements of Channel 157 are pretty noisy, while the rest is still clearly distinguishable enough for different activities. \emph{This implies the wide bandwidth has potentials for the RFI robustness.} We zoom in Fig.~\ref{fig:examplefrequencyresponsenoisewhole} and look at the CSI vectors in the same bandwidth of 5.8 GHz 802.11 Channel 157, which is shown in Fig.~\ref{fig:examplefrequencyresponsenoisepart}. It is clearly shown that RFI changes the pattern of large percentage of CSI vectors at all, and impossible to explore any pattern for those CSI vectors. However, when looking at the big picture of the CSI vectors, certain percentage of the CSI vectors for each activity have the same pattern. This means \emph{utilisation of a group of CSI samples also have feasibility for recognition under RFI}.  

%XXX
%
%Therefore, for activities under RFI, there are two ways to be robust to RFI. Firstly, the wider bandwidth is used for distinguishing the activity under RFI. However, if only interfered bandwidth is available, multiple CSI vectors can be explored for making the final decision. However, there is a question \emph{what method is the best for making decision by using multiple CSI vectors}. The most intuitive method is majority voting. Moreover, we proposed a weighting fusion method using $\ell_1$ minimisation and show the superiority in different experiment settings. We will further discuss this in Section \ref{subsec:secondtier} and Section \ref{sec:experiments}.
%
%To sum up, \emph{these facts implies that SNR has potentials for walking detection without RFI, but not informative enough for static activity recognition and SNR even does not take effect for walking detection under RFI. CSI is more sensitive and informative to different kinds of activities, and also potentially robust to RFI.} 




\subsection{Activity Recognition with RFI}
\label{subsec:ar_with_rfi}

We now describe our proposed CSI-based activity recognition in the presence of RFI. The goal of activity recognition is to identify four daily activities: sitting, standing, lying and walking, as well as whether the AoI is empty. 


\subsubsection{Data collection and pre-processing ???}

Our method fingerprints the activities using CSI vectors. The first procedure is to record the CSI vectors for building a training set, and use the training set to fingerprint the test data by using our proposed machine learning method. The machine learning method we use is optimised sparse representation classification (SRC). As the main superiority of SRC is featureless, we use CSI vectors of all the activities in the dictionary. 


For each CSI vector, we first apply Exponential smoother to remove the high frequency noise and decrease the noise level. However, Exponential smoother cannot take effect for all the cases when SNR is high, we still need further mechanism to improve the performance.

There are several advantage of SRC method. First, SRC can use samples directly for classification, do not have to perform feature selection. This allows the CSI vector can be directly used for fingerprinting, do not need to consider the which features of CSI vector are best activity recognition. Second, SRC is known as being robust to the noise. As our research work is to investigate the performance of activity recognition under RFI, we investigate how to explore SRC to increase SNR for improving activity recognition.

When building a dictionary. The most obvious method is to put training samples to the training set. However, RFI may cause the unexpected change to CSI vectors. There is no existing model for the performance of CSI vector under RFI. Therefore, we need to consider the RFI environment when training the dictionary. In other words, the CSI vectors of one specific activity under different physical environment and radio environment vary. We have to perform training for the new environment. The method in \cite{wang2014eyes} can be applied for updating the dictionary for RFI environment.


%The aim of our system is to perform a multi-class classification for accurately recognising four normal activities in daily life, i.e. . The system also tell whether the AoI is empty.

%In our method, there are two main tasks for activity classification. The first task is for distinguish the walking status and \emph{static status}, and the goal of the second task is for classifying specific static activity. 

%As introduced the challenge that activity recognition under RFI is considered in the paper. During the classification process, we proposed optimised fusion method to improve the performance for the activity recognition under RFI.

%There are two tiers for the recognition system. The first tier is to distinguish the walking status from static status, while the task of the second tier is to classify the specific static activity.

%The reason to divide the method into two tiers is the variety of the walking status. 


%Unlike the static status, walking status cause different interference condition while moving. 
%We can apply the same method for walking detection as the static activities. Since some CSI of walking status may have the similar pattern with the static status. This may cause \emph{false negatives} or \emph{false positives} for activities recognition. Alternatively, we can use the deviation of CSI vectors in one specific length window to make a decision for walking detection.  Therefore, it is suggested to divide the recognition method into walking detection and static activity recognition. The similar mechanisms are also discussed in the previous state-of-the-art \cite{wang2014eyes}\cite{sigg2014rf}. Intuitively, the variance of walking status in a window is greater than the that of the static ones. Therefore, we can abstract features to distinguish between the walking status and the static status. We also optimised the method to select the best subcarriers for walking detection. However, this mechanism has some limitation under RFI. Deviation based features is not robust to RFI. We will further discuss the efficiency and limitation in Section \ref{subsec:WalkingDetection}.

%There are three steps for the second tier the activity recognition, this system uses finger-print methods for the activity recognition, so the first step is off-line dictionary training, the second step is to on-line perform the activity recognition. 


%\subsection{Shape-based Signal-to-Noise Radio~(SSNR)}
%
%\begin{figure}[htb]
%   \centering
%    \includegraphics[scale = 0.35]{figure/SSNR_example/SSNR_example.eps}
%    \caption{The example of CSI amplitude without/ under interference}\label{fig:SSNR_example}
%\end{figure}
%% SSNR feature
%To meet the challenge of activity recognition under RFI, we need to consider one question \emph{how to estimate CSI of one signal is noisy or not}.
%
%We propose \emph{Shape-based Signal-to-Noise Radio~(SSNR)} for activity recognition to show the noise level. As shown in Fig.~\ref{fig:SSNR_example},
%the change of the amplitude of continuous elements of CSI amplitude vectors is small when there is no interference, so it can be seen as continuous function. However, it changes dramatically in which subcarriers the radio interference happens.  For example, the radio interference happens from 120th subcarrier to 220th subcarrier in Fig.~\ref{fig:SSNR_example}.
%
%Intuitively, compared with the smooth change of the elements in the CSI amplitude vector, the interference will cause relative high frequency change. We can take advantage of this to abstract the relative ratio of the energy between the smooth and the discontinuous signal. Technically, this is not Signal-to-Noise Ratio~(SNR), the energy of the messy subcarriers includes the energy of the signal as well as the noise. Since the characteristic is calculated based on the shape, we call this feature as Shape-based Signal-to-Noise Radio~(SSNR). 
%
%We calculate SSNR using the ratio between the energy of the low frequency  and that of the high frequency in Equ.~\ref{eqn:ssnr}. 
%\begin{equation}
%SSNR(C_i) = 20log_{10} \frac{rms (low(E(C_i)))}{rms(high(E(C_i)))}    \label{eqn:ssnr}
%\end{equation}
%$fr_i$ is the CSI amplitude vector for $i$-th sample. $rms$ is root mean square. As the ratio of many CSI amplitude vectors has wide dynamic range, we choose to express it as the logarithmic decibel scale.  
%
%\begin{equation}
%low(E(C_i)) = \{a_{ij}\} ~~~ j <= id   \label{eqn:low}
%\end{equation}
%\begin{equation}
%high(E(C_i)) = \{a_{ij}\} ~~~ j >id   \label{eqn:high}
%\end{equation}
%
%$a_{ij}$ is the energy distribution for $j$-th bin for the $i$-th sample after Fast Fourier Transformation~(FFT) calculation for $fr_i$. $id$ is the threshold to decide the high frequency and low frequency.
%
%Fig.~\ref{fig:SNR_vec} shows the SSNR of CSI amplitude vectors in Fig.\ref{fig:examplefrequencyresponse}. In our method, there are two usages in our paper. First, SSNR is used for determining the walking status. Second, SSNR is for weighting the coefficients from $\ell_1$ minimisation to boosting SNR~(details discussed in Section~\ref{subsec:CoefficientFusion} ). 
%
%\begin{figure}[htb]
%   \centering
%    \includegraphics[scale = 0.35]{figure/Example_frequency_response/Example_SSNR.eps}
%    \caption{The example of SSNR}\label{fig:SNR_vec}
%\end{figure}
%
%Two situations can cause the variance of SSNR in short time. One is the variance of signal energy which happens in walking status, and the other one is the variance of the noise energy caused by radio frequency interference. Fig.~\ref{fig:exampleSSNR2situations}) shows the example of the SSNR stability in static status and the SSNR variance caused by RFI and walking status. This also demonstrates the two usages of SSNR, the SSNR variance cause by walking status can help to detect the walking status, while as shown in Fig.~\ref{fig:SSNR_example}, the CSI vector without RFI have more informative subcarriers, which characteristic we utilise to weight for the final decision. Details are discussed in Section~\ref{subsec:firsttier}.
%
%\begin{figure}[ht]
%{
%\centering
%       \subfigure[CSI amplitute vector in Clean environment]{
%        \includegraphics[scale = .35]{figure/SSNR_2_situations/example_2_situation_frequency_response.eps}
%        \label{fig:exampleSSNRwalking}
%    }
%    \subfigure[SSNR]{
%        \includegraphics[scale = .35]{figure/SSNR_2_situations/example_2_situation_ssnr.eps}    
%        \label{fig:exampleSSNRinterference}
%        }
%         
%         \caption{Frequency response and SSNR performance in different activities}
%               \label{fig:exampleSSNR2situations}               
%}
%\end{figure} 

% \subsection{Exponential Smoothing}

%\subsection{Walking Detection}\label{subsec:firsttier}
%As discussed in the previous works \cite{wang2014eyes}\cite{sigg2014rf}. Deviation feature based walking detection is intuitive and popular. In this section, we discuss the deviation feature based walking detection and proposed an optimised method to select the best continuous subcarriers for walking detection. We also introduce the limitation of the deviation feature based walking detection, and show more details in Section \ref{sec:experiments}.
%As shown in \ref{fig:exampleRSS}, SNR shows larger deviation when the monitored person is walking. We take advantage of this characteristic for walking detection.
%
%The aim of walking detection is to classify the monitored object is static or walking. In our work four features of deviation of SNR are used show in the Table \ref{features}, where $S$ is the SNR vector in window, $\mu$ is the mean value of $S$.   
%
%\begin{table}
%    \begin{tabular}{|l|l|}
%        \hline
%        Feature                  & Equation \\ \hline
%        Standard Deviation       &  $\sigma = \frac{1}{n-1}  \sqrt{ E[( S(k)- \mu )^2]  }$         \\ \hline
%        Peak                     & $\rho = max ( S ) - min ( S )$          \\ \hline
%        Head Size                & $\eta = max ( S ) - median ( S )$        \\  
%        \hline
%        3rd Order Central moment & $\gamma = E[(S(k)- \mu)^3 ] $        \\ \hline
%    \end{tabular}\label{features}
%    \caption{Features for walking detection}
%\end{table}
% 
%%The first feature is named \emph{Peak} which calculates the difference between the maximum value and the minimal value in one window with size $w$. 
%%
%%\begin{equation}
%% \rho  = max ( S(1),S(2),...,S(w) ) - min ( S(1),S(2),...,S(w) )     \label{eqn:peakfeature}
%%\end{equation}
%%where $max$ and $min$ are the operator which gets the maximum and minimal value in a vector. $S(i)$ is SNR of $i$-th sample.
%%
%%We also propose a new feature named \emph{Head-size} which calculates the difference between the maximum value and the median value in one window.
%%\begin{equation}
%% \eta   = max ( S(1),S(2),...,S(w) ) - median ( S(1),S(2),...,S(w) )     \label{eqn:headsize}
%%\end{equation}
%%where $median$ get the median value of a vector.
%%% % TODO : use mode instead of median ?
%
%For the feature based machine learning method, it is always challenging to select the best feature. Using all the features is not necessarily best for the decision making. Moreover, the best features for one dataset is not always good choice for other dataset. To diminish the performance influence from features, we selecting features sequentially using the training set until no performance increases. When selecting features, we use 10 cross validation. As the walking detection is binary classification, we need to consider both true positive rate and false positive rate, so we use f1 score as criterion for feature selection. As discussed, the selected best features for one training set is not necessarily best for the other ones, we suggest the method use for dynamic feature selection, i.e. conducting feature selection for each training set. 
%
%%From Fig.\ref{fig:exampleRSS}, the walking status cause relatively high variety of SNR compared with the static status. However, the RFI also causes high \emph{Peak} value. In some cases, the \emph{Peak} value of SNR in RFI even higher than that of walking status, which cause False Positive~(FP) for detecting the walking status. Therefore \emph{Head-size} feature is introduced. There is one clear difference between the SNR under RFI and walking status. In most of the cases, RFI cause the decrease of SNR, because the relative energy of noise is high during RFI. On the contrary, it can change the energy of signal because of the interference of the person in different position during walking. Therefore, the SNR under walking status varies dramatically instead of only decreasing. \emph{Head-size} feature can show the characteristic. Standard deviation works fine in the situation without RFI, but it takes no effect during RFI as RFI also can cause high deviation which hardly shows the difference between the walking status and the static status with RFI. In walking detection, we use \emph{Peak} and \emph{Head-size} feature for detecting the walking status.
%
%As walking detection is binary classification, we choose to use the logistic regression model for classification.
%
%\begin{equation}
%S(F) =  \frac{1}{1+e^{-( \alpha_{0} + \sum {\alpha_{k} F(k) } )} }   =\begin{cases}0 & static\\1 & walking\end{cases}   \label{eqn:logisticmodel}
%\end{equation}
%where $F$ are feature set of SNR for a fixed window size and $S(F)$ is the function to determine the walking status or not. 
%
%% choose part of subcarriers to make decision
%When the large number of subcarriers are available, the performance of using more subcarriers is not necessary better. We can choose part of bandwidth along with feature selection for walking detection. 
%
%To choose part of bandwidth, we need to use a criterion to evaluate the fit goodness of the posterior estimation. The residual is to see the fit goodness of the logistic regression. The definition of residual for a logistic mode is Equ.\ref{eqn:pearsonresidual} 
%
%\begin{equation}
%r_{i} =  y_{i}-   \hat{y_i} , i = 1,2,...,n
%  \label{eqn:pearsonresidual}
%\end{equation}
%
%$y_i$ is the $i$-th observed result, and $\hat{y_i}$ is the $i$-th predicted result. $n$ is the size of training set. Then we use a factor Root Mean Square $g$ to show the fitting goodness of the training set, where $g = rms(r_1, r_2, ... , r_n)$.
% 
%
%We set an offset and greedy search for the minimal $g$ using different numbers of continuous subcarriers and different part of continuous subcarriers, and use these continuous subcarriers for walking detection. 
%
%Alternatively, as walking also causes the similar pattern, we can use $\ell_1$ method for detecting walking. The aim of abstracting the walking status out is the variety caused by walking. The walking is dynamic and the CSI vector caused by the walking may have the same pattern as the other static activities. Therefore, it is more accurate for walking detection according to the deviation and cause less false negatives for the static activity recognition. However, there is limitation of the walking detection according to the deviation based features. \emph{RFI also introduces the SNR deviation, so this characteristic may be difficult or not feasible for walking detection if there is not available continuous subcarriers for our optimised method to select.} We will discuss in Section \ref{sec:experiments} to compare the accuracy of walking detection by using deviation features and $\ell_1$ method directly.



%In the Second Tier, only the identified static activities are sent to the second tier. 



%Fig.~\ref{eqn:headsize} shows the CSI amplitude vectors in different RFI environments.
%For visual clarity, we only shows the CSI amplitude vectors of 10 samples.
%\begin{figure}[htb]
%   \centering
%    \includegraphics[scale = 0.35]{figure/example_RFI_training/CSI_amp.eps}
%    \caption{CSI amplitude vectors under different RFI situations}\label{fig:example_RFI_training}
%\end{figure}

%% get rid of the noisy samples
%When adding the training sample under the signal interference, the noise-dominant samples are introduced as well. If the CSI amplitude vectors are noise-dominant, we cannot tell the difference among the several classes. The energy difference of the noise-dominant CSI amplitude vectors is mainly due to the RFI rather than the activity. 
%
%Therefore, we cannot use the noise-dominant CSI amplitude vectors for training. To clean the dictionary, we put all the noisy samples in one class, i.e we also have one class in the training for noise-dominant CSI amplitude vectors except the static status.
%
%We suggest a method to determine the noisy samples according to SSNR. Intuitively, the value of SSNR of the noise-dominant CSI amplitude vectors are lower than the that of the normal CSI amplitude vectors in one class.
%
%Our method is to set a threshold for each class of signals. If the SSNR of one signal is below the threshold, it will be recognised as the noisy signal. The threshold we use is
%\begin{multline}
%SSNRthreshold_i =   median(s_{i1}, ...,s_{ic_i}) \\
%-  coe * ( median(s_{i1}, ...,s_{ic_i}) \\
% - min(s_{i1}, ...,s_{ic_i}) ) ,  0<= coe < 1 \label{eqn:logisticmodelSSNRthreshold}
%\end{multline} 
%$s_{ij}$ is the $j$-th SSNR value for the $i$-th class. 
%
%% dictionary cleaning similar columns (This part is decided yet)
%After the dictionary gets rid of the noisy columns, we need to consider the coherence of the frequency response in each class. As the activities classified by tier two are static, the dissimilarity of the columns among each classes are very important. If a column in one class is more similar to one other class, the column should be taken away from the training set.
%
%In the step, we take advantage of Leave-one-out cross-validation (LOOCV). For each training sample of the static status. We calculate the coherence between it and other training samples of static status, and use $k$ nearest neighbour method to make a decision. If the class of the final decision is not the same as the class that training sample belongs to, this training sample is deleted from training set.  

% dictionary reduction (delete)
%\subsection{Classifiers chosen} \label{subsec:classiferschosen}
%Sparse representation shows the priority in noisy environment. For static status classification, we choose to use $\ell_1$ minimisation to improve the accuracy. We already have a dictionary with $s$ classes $D = \{d_{11},...d_{1n_{i}},...d_{i1},...,d_{in_{i}}...,d_{s1},...,d_{sn_{s}} \}$. 
%The test sample of $y$ can be expressed by the dictionary $D$ with coefficient vector $x$, i.e. $y = Dx$. Due to the noise $n$, $x$ cannot exactly expressed by the Dictionary $D$. Wright etc. \cite{Wright:09} suggest to solve $x$ by using 
%\begin{equation}
%\hat{x} = \argmin_x \| x \|_1 \quad \text{ subject to } \|y - Dx\|_2 < \epsilon,
%\label{eqn:l1minimization}
%\end{equation}
%where $\epsilon$ stands for the noise.


\subsubsection{Classification algorithms} 
\label{subsec:CoefficientFusion}
We have seen that RFI causes the CSI vector to be very noisy. In order to deal with CSI, we introduce a window size $ws$ where $ws$ consecutive CSI vectors are used for classification. One possible method is to stack $ws$ CSI vectors into a tall feature vector and use it for classification. However, this will be computation intensive because the feature vector has a very high dimension. Instead, we will use the $ws$ one at a time and investigate different fusion methods. 

Let $y_1, y_2, ..., y_{ws}$ denote the CSI vectors in the time window, and $D$ be the dictionary. We first solve the following $\ell_1$-optimisations for $i = 1,.., ws$: 
\begin{equation}
\hat{x}_i = \argmin_x \| x \|_1 \quad \text{ subject to } \|y_i - Dx\|_2 < \epsilon,
\label{eqn:l1minimization}
\end{equation}

We now present three different fusion methods which use $\hat{x}_i$ ($i = 1,.., ws$) in different ways. 

The first method is to use decision fusion and will be referred to as $\ell_1 \; voting$. For this method, the algorithm uses each $\hat{x}_i$ to arrive at a decision class using the standard SRC algorithm described in Section \ref{subsec:sparseapproximation}. This method then uses majority voting to arrive at a decision. 

The second method is to fuse the $\hat{x}_i$ vectors by computing their mean: $\hat{x}_{\rm sumup} = \frac{1}{ws} \sum_{i = 1}^{ws} \hat{x}_i$. The mean vector $\hat{x}_{\rm sumup}$ is then use to compute the residuals for each class as in the standard SRC algorithm described in Section \ref{subsec:sparseapproximation}. This method returns the class that minimises the residual. Note that this fusion method was proposed by Misra et al.~in \cite{misra2014energy} where they shown that such method could improve the GPS recovery accuracy. We will call this method \emph{$\ell_1$ sumup}.

The method \emph{$\ell_1$ sumup} applies equal weights to all $\hat{x}_i$ by computing a simple average of them. However, it is possible that some CSI vectors in the window are less affected by noise. This can also be seen from Fig.~\ref{fig:dynamicRSSexample} where the SNR fluctuates. We therefore propose to use SNR of a sample to derive a weighting for that sample. Let $S_i$ denote the SNR of the $i$-th sample in the window. We compute the weighted mean of $\hat{x}_i$ using: 
\begin{equation}
\hat{x}_{\rm weighting}  =  \sum {w_{i}} \hat{x}_i ,
\label{eqn:weighting}
\end{equation}
\begin{equation}
w_i =  \frac{A_i}{ \sum_{j = 1}^{ws} {A_j} }, \quad   A_i = 10^{( \frac{S_i}{20} )},
\label{eqn:weightingelement}
\end{equation}

The mean vector $\hat{x}_{\rm weighting}$ is then use to compute the residuals for each class as in the standard SRC algorithm described in Section \ref{subsec:sparseapproximation}. This method returns the class that minimises the residual. We call this method as \emph{$\ell_1$ weighting}. 



 

%Here is questions that \emph{how to make final decision according to the CSI vectors within the window size}. The most obvious way is majority voting. The method using one CSI vector fails to determine some CSI amplitude samples because of random and unpredictable elements, like RFI noise, but the features in one class still should be similar to each other, which mean statistically most of the test samples in one class should be classified correctly. This is the basic principle of the majority voting. 

%Besides this, we propose an optimised method for the result fusion according to the coefficients from $\ell_1$ minimisation (Equ. (\ref{eqn:l1minimization})). 
%First, we can use the same mechanism that calculate the mean of coefficients and test CSI vectors in one window and use mean of them to calculate the residuals, and also select the class with the minimal one as final decision. We call this method as \emph{$\ell_1$ sumup}.
%
%Alternatively, we can calculate weighted arithmetic mean of the coefficients returned from the sparse representation. In one window the RFI bring noise to certain percentage of CSI samples. If simply adding the coefficient vector, it also brings the noise into the consideration for make decision. If not adding some CSI samples below a certain threshold, it may miss some useful information and it is also not easy to decide which threshold is suitable to decide the CSI amplitude vector is noisy or not. Considering those issues, we use weight to get the summation. 
%
%The weighting approach is based on the SNR we propose. For the static activity, the movement is still and the RFI is the main factor to cause the SNR variance. This means higher the SNR level indicates is more informative then the lower one, and should be weighted more. The weight method is show in Equ.~(\ref{eqn:weighting})
%\begin{equation}
% \tilde{x}  =  \sum {w_{i}} \hat{x}_i ,
%\label{eqn:weighting}
%\end{equation}
%\begin{equation}
%w_i =  \frac{A_i}{ \sum_{j = 1}^{ws} {A_j} }, \quad   A_k = 10^{( \frac{S(k)}{20} )},
%\label{eqn:weightingelement}
%\end{equation}
%
%And then the modified SRC method is utilised to make the final decision. Instead of using one CSI sample vector, we calculate the weighted mean value of the CSI sample vectors in one window size, i.e. $ \overline{y} = \sum_{j=1}^{ws} {{w_i}{y_i}} $, and calculate the residual for $i$-th class by $ \tilde{r_i} =  \|{\overline{y} - D\tilde{x}_i}\|_{2}$. The final step is also to select the class with the minimal residual as the final decision. We call this method as \emph{$\ell_1$ weighting} 
%
%



